Misalignment-Robust Frequency Distribution Loss for Image Transformation

This paper aims to address a common challenge in deep learning-based image transformation methods, such as image enhancement and super-resolution, which heavily rely on precisely aligned paired datasets with pixel-level alignments. However, creating precisely aligned paired images presents significant challenges and hinders the advancement of methods trained on such data. To overcome this challenge, this paper introduces a novel and simple Frequency Distribution Loss (FDL) for computing distribution distance within the frequency domain. Specifically, we transform image features into the frequency domain using Discrete Fourier Transformation (DFT). Subsequently, frequency components (amplitude and phase) are processed separately to form the FDL loss function. Our method is empirically proven effective as a training constraint due to the thoughtful utilization of global information in the frequency domain. Extensive experimental evaluations, focusing on image enhancement and super-resolution tasks, demonstrate that FDL outperforms existing misalignment-robust loss functions. Furthermore, we explore the potential of our FDL for image style transfer that relies solely on completely misaligned data. Our code is available at: https://github.com/eezkni/FDL

==> figures/DIV2K_comparison.tex <==
\begin{figure*}[t]
    \centering 
    \subfloat[LR]{
    \begin{minipage}[b]{0.16\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/053_x2/LR.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/077_x2/LR.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/079_x2/LR.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/092_x2/LR.png}
    \end{minipage}
    }
    \subfloat[GT]{
    \begin{minipage}[b]{0.16\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/053_x2/GT.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/077_x2/GT.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/079_x2/GT.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/092_x2/GT.png}
    \end{minipage}
    }
    \subfloat[LPIPS]{
    \begin{minipage}[b]{0.16\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/053_x2/LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/077_x2/LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/079_x2/LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/092_x2/LPIPS.png}
    \end{minipage}
    }
    \subfloat[PDL]{
    \begin{minipage}[b]{0.16\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/053_x2/PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/077_x2/PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/079_x2/PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/092_x2/PDL.png}
    \end{minipage}
    }
    \subfloat[Contextual Loss]{
    \begin{minipage}[b]{0.16\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/053_x2/CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/077_x2/CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/079_x2/CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/092_x2/CX.png}
    \end{minipage}
    }
    \subfloat[FDL(ours)]{
    \begin{minipage}[b]{0.16\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/053_x2/ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/077_x2/ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/079_x2/ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DIV2K/092_x2/ours.png}
    \end{minipage}
    }
    \hfill
    % \vspace{-5pt}
	\caption{
		Qualitative results on DIV2K dataset~\cite{DIV2K} and NLSN~\cite{meiImageSuperResolutionNonLocal2021}. We randomly shifted the HR images before down-sample it into LRs. Zoom in to observe details.
	}
    % \vspace{-15pt}
	\label{fig:DIV2k_comparison}
\end{figure*}

==> figures/DIV2K_shift.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.98\linewidth]{imgs/supply/DIV2K.drawio.pdf}
\caption{
Process of creating a dataset with random misalignment based on the DIV2K~\cite{DIV2K}.
}
% \vspace{-10pt}
\label{fig:DIV2K_shift}
\end{figure}

==> figures/DPED_comparison.tex <==
\begin{figure*}[t]
    \centering 
    \subfloat[Low Quality]{
    \begin{minipage}[b]{0.2\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/8/8.jpg}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/15/15.jpg}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/27/27.jpg}
    \end{minipage}
    }
    \subfloat[LPIPS]{
    \begin{minipage}[b]{0.2\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/8/LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/15/LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/27/LPIPS.png}
    \end{minipage}
    }
    \subfloat[PDL]{
    \begin{minipage}[b]{0.2\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/8/PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/15/PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/27/PDL.png}
    \end{minipage}
    }
    \subfloat[Contextual Loss]{
    \begin{minipage}[b]{0.2\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/8/CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/15/CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/27/CX.png}
    \end{minipage}
    }
    \subfloat[FDL(ours)]{
    \begin{minipage}[b]{0.2\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/8/ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/15/ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/comparison/DPED/27/ours.png}
    \end{minipage}
    }
    \hfill
    % \vspace{-5pt}
	\caption{
		Qualitative results on DPED dataset~\cite{ignatovDSLRQualityPhotosMobile2017a} and NAFNet~\cite{chen2022simple} compared with LPIPS, PDL, CTX. The red area is cropped
from different results and enlarged for visual convenient. Zoom in to observe details.
	}
    % \vspace{-15pt}
	\label{fig:DPED_Comparison}
\end{figure*}

==> figures/DPED_misalign.tex <==
\begin{figure}[t]
    \centering 
    \subfloat[GT]{
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/DPED_unalign/GT/0.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/DPED_unalign/GT/1.png}
    \end{minipage}
    }
    \subfloat[LQ]{
    \begin{minipage}[b]{0.24\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/DPED_unalign/LR/0.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/DPED_unalign/LR/1.png}
    \end{minipage}
    }
    % \vspace{-6pt}
    \hfill
	\caption{
    An example of noticeable geometric misalignment within image pairs from the DPED dataset.
	}
    % \vspace{-10pt}
	\label{fig:DPED_misalign}
\end{figure}

==> figures/SR_comparison.tex <==
\begin{figure*}[t]
    \centering 
    \subfloat[GT]{
    \begin{minipage}[b]{0.32\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/SR/HR.png}
    \end{minipage}
    }
    \subfloat[L1]{
    \begin{minipage}[b]{0.32\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/SR/L1.png}
    \end{minipage}
    }
    \subfloat[FDL (Ours)]{
    \begin{minipage}[b]{0.32\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/SR/FDL.png}
    \end{minipage}
    }
    % \vspace{-6pt}
    \hfill
	\caption{
    Qualitative comparison results of NLSN~\cite{mei2021image} on our synthetic shifted DIV2K dataset. Training a model using L1 loss results in regression to the mean phenomenon. In contrast, FDL exhibits misalignment robustness, ensuring the overall quality of predicted images in misaligned scenarios.
	}
    % \vspace{-12pt}
	\label{fig:SR_comparison}
\end{figure*}

==> figures/SWD.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.0
\linewidth]{imgs/framework/SWD.pdf}
\vspace{-8mm}
\caption{
An example of the patch-level Sliced Wasserstein Distance.
%
PDL~\cite{delbracioProjectedDistributionLoss2021} can be considered as a special case of $P=1$.
}
\label{fig:SWD}
\end{figure}

==> figures/autoencoder_reconstruct.tex <==
\begin{figure}[tb]
    \centering 
    \subfloat[origin]{ \includegraphics[width=0.16\textwidth]{imgs/toy_example/frequency_component/autoencoder_origin.png}}
    \subfloat[low frequency]{ \includegraphics[width=0.16\textwidth]{imgs/toy_example/frequency_component/autoencoder_low_frequency.jpeg}}
    \subfloat[high frequency]{ \includegraphics[width=0.16\textwidth]{imgs/toy_example/frequency_component/autoencoder_high_frequency.jpeg}}
    \hfill
    % \vspace{-5pt}
	\caption{
		A toy example illustrates the image information characterized by VGG features with different frequencies with auto-encoder: A corresponding decoder is used to reconstruct the image for each frequency component. a) original image, b) reconstruction using only the low-frequency component, and c) reconstruction using only the high one.
	}
    % \vspace{-15pt}
	\label{fig:autoencoder_reconstruct}
\end{figure}

==> figures/headline.tex <==
\begin{figure*}[t]
    \centering 
    \subfloat[Ground Truth]{
    \begin{minipage}[b]{0.321\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/headline/gt.png}
    \end{minipage}
    }
    \subfloat[LPIPS]{
    \begin{minipage}[b]{0.16\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/headline/LPIPS_1.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/headline/LPIPS_2.png}
    \end{minipage}
    }
    \subfloat[PDL]{
    \begin{minipage}[b]{0.16\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/headline/PDL_1.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/headline/PDL_2.png}
    \end{minipage}
    }
    \subfloat[CTX]{
    \begin{minipage}[b]{0.16\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/headline/cx_1.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/headline/cx_2.png}
    \end{minipage}
    }
    \subfloat[FDL (Ours)]{
    \begin{minipage}[b]{0.16\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/headline/ours_1.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/headline/ours_2.png}
    \end{minipage}
    }
    \hfill
    % \vspace{-5pt}
	\caption{
		Qualitative results on DPED dataset~\cite{ignatovDSLRQualityPhotosMobile2017a} and NAFNet~\cite{chen2022simple} compared with LPIPS, PDL, CTX. The red area is cropped
from different results and enlarged for visual convenient. Zoom in to observe details.
	}
    % \vspace{-15pt}
	\label{fig:DPED_Comparison}
\end{figure*}

==> figures/supply/DIV2K_comparison.tex <==
\begin{figure*}[ht]
    \centering 
    \vspace{-24pt}
    \subfloat[LPIPS]{
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img017_x2_SR_LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img054_x2_SR_LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img056_x2_SR_LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img077_x2_SR_LPIPS.png}
    \end{minipage}
    }
    \subfloat[PDL]{
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img017_x2_SR_PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img054_x2_SR_PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img056_x2_SR_PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img077_x2_SR_PDL.png}
    \end{minipage}
    }
    \subfloat[CTX]{
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img017_x2_SR_CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img054_x2_SR_CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img056_x2_SR_CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img077_x2_SR_CX.png}
    \end{minipage}
    }
    \subfloat[FDL (Ours)]{
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img017_x2_SR_ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img054_x2_SR_ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img056_x2_SR_ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DIV2K/img077_x2_SR_ours.png}
    \end{minipage}
    }
    \vspace{-6pt}
    \hfill
	\caption{
		Qualitative comparison of SISR using the NLSN model~\cite{mei2021image} trained with synthetic shifted DIV2K dataset, compared with LPIPS~\cite{zhangUnreasonableEffectivenessDeep2018}, and PDL~\cite{delbracioProjectedDistributionLoss2021}, 
    and CTX~\cite{mechrezContextualLossImage2018}. The red area is cropped from different results and enlarged for visual convenient. Zoom in to observe details.
	}
	\label{fig:supply_DIV2K_Comparison}
\end{figure*}



==> figures/supply/DPED_comparison.tex <==
\begin{figure*}[ht]
    \centering 
    \vspace{-12pt}
    \subfloat[LPIPS]{
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/0_LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/10_LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/18_LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/20_LPIPS.png}
    \end{minipage}
    }
    \subfloat[PDL]{
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/0_PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/10_PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/18_PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/20_PDL.png}
    \end{minipage}
    }
    \subfloat[CTX]{
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/0_CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/10_CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/18_CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/20_CX.png}
    \end{minipage}
    }
    \subfloat[FDL (Ours)]{
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/0_ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/10_ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/18_ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/DPED/20_ours.png}
    \end{minipage}
    }
    \vspace{-6pt}
    \hfill
	\caption{
		Qualitative results of image enhancement using NAFNet~\cite{chen2022simple} trained with the DPED dataset~\cite{ignatovDSLRQualityPhotosMobile2017a}.
	}
    % \vspace{-12pt}
	\label{fig:supply_DPED_Comparison}
\end{figure*}


==> figures/supply/REALSR_comparison.tex <==
\begin{figure*}[ht]
    \centering 
    \vspace{-12pt}
    \subfloat[LPIPS]{
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/001_LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/007_LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/022_LPIPS.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/028_LPIPS.png}
    \end{minipage}
    }
    \subfloat[PDL]{
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/001_PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/007_PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/022_PDL.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/028_PDL.png}
    \end{minipage}
    }
    \subfloat[CTX]{
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/001_CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/007_CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/022_CX.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/028_CX.png}
    \end{minipage}
    }
    \subfloat[FDL (Ours)]{
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/001_ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/007_ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/022_ours.png}
        \\
        \includegraphics[width=1.0\textwidth]{imgs/supply/comparison/REALSR/028_ours.png}
    \end{minipage}
    }
    \vspace{-6pt}
    \hfill
	\caption{
		Qualitative comparison of real-world SISR using the NAFNet~\cite{chen2022simple} trained with the merged real-world dataset~\cite{cai2019toward, chen2019camera}.
	}
    % \vspace{-12pt}
	\label{fig:supply_REALSR_Comparison}
\end{figure*}

==> figures/supply/style_comparison.tex <==
\begin{figure*}[ht]
    \centering 
    \begin{minipage}[b]{1.0\textwidth}   
        \hfill
        \centering
        \begin{minipage}[c]{0.25\textwidth}
        \end{minipage}
        \hfill
        \begin{minipage}[c]{0.73\textwidth}
            \hspace{0.35pt}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/styles/brick.png}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/styles/cycle.png}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/styles/mosaic.jpeg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/styles/picasso.jpeg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/styles/triangle.png}
            \hfill
            \\
            \rotatebox{0}{\small{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~Style Images~~~~~~~~}}
        \end{minipage}
    \end{minipage}
    \vspace{4pt}
    \\
    \centering
    \begin{minipage}[b]{1.0\textwidth}
        \hfill
        \begin{minipage}[c]{0.25\textwidth}
            \centering
            \vfill
            \includegraphics[width=1.0\textwidth]{imgs/supply/style_transfer/bridge/bridge.png}
            \rotatebox{0}{\small{~~~~~~~~Content Image~~~~~~~~}}
            \vfill
        \end{minipage}
        \hfill
        \begin{minipage}[c]{0.73\textwidth}
        \subfloat[Gatys \etal]{
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/origin/brick.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/origin/cycle.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/origin/mosaic.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/origin/picasso.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/origin/triangle.jpg}
        }
        \vspace{-8pt}
        \\
        \subfloat[CTX]{
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/CTX/brick.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/CTX/cycle.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/CTX/mosaic.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/CTX/picasso.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/CTX/triangle.jpg}
        }
        \vspace{-8pt}
        \\
        \subfloat[FDL]{
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/ours/brick.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/ours/cycle.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/ours/mosaic.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/ours/picasso.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/bridge/ours/triangle.jpg}
        }
        \end{minipage}
    \end{minipage}
    \\
    \addtocounter{subfigure}{-3}
    \centering 
    \begin{minipage}[b]{1.0\textwidth}
        \hfill
        \begin{minipage}[c]{0.25\textwidth}
            \centering
            \vfill
            \includegraphics[width=1.0\textwidth]{imgs/supply/style_transfer/chtholly/chtholly.jpeg}
            \rotatebox{0}{\small{~~~~~~~~Content Image~~~~~~~~}}
            \vfill
        \end{minipage}
        \hfill
        \begin{minipage}[c]{0.73\textwidth}
        
        \subfloat[Gatys \etal]{
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/origin/brick.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/origin/cycle.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/origin/mosaic.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/origin/picasso.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/origin/triangle.jpg}
        }
        \vspace{-8pt}
        \\
        \subfloat[CTX]{
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/CTX/brick.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/CTX/cycle.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/CTX/mosaic.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/CTX/picasso.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/CTX/triangle.jpg}
        }
        \vspace{-8pt}
        \\
        \subfloat[FDL (Ours)]{
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/ours/brick.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/ours/cycle.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/ours/mosaic.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/ours/picasso.jpg}
            \includegraphics[width=0.19\textwidth]{imgs/supply/style_transfer/chtholly/ours/triangle.jpg}
        }
        \end{minipage}
    \end{minipage}
    \\
    \hfill
	\caption{
		Qualitative results of style transfer compared with Gatys \etal and CTX. 
	}
	\label{fig:supply_style_Comparison}
\end{figure*}

==> tables/Ablation_patch.tex <==
\begin{table}[htp]
    \centering
    % \resizebox{\linewidth}{!}{
    % \small
    \footnotesize
    \renewcommand\arraystretch{1.0}
    \setlength{\tabcolsep}{2.2pt}
    \caption{Ablation of patch size.}
    \begin{tabular}{c|cccccc}
    % \toprule
    \hline
    \hline
    Patch size  & PSNR$\uparrow$ & LPIPS(VGG)$\downarrow$ & DISTS$\downarrow$ & SSIM$\uparrow$  & FID$\downarrow$ \\
    \midrule
    1     & 22.994 & 0.116 & 0.122 & 0.810 & \textcolor[rgb]{ 1,  0,  0}{24.599} \\
    3     & 23.041 & 0.117 & 0.123 & 0.807 & 31.886 \\
    6     & 22.992 & 0.118 & 0.125 & 0.797 & 41.174 \\
    \midrule
    5     & \textcolor[rgb]{ 1,  0,  0}{23.048} & \textcolor[rgb]{ 1,  0,  0}{0.114} & \textcolor[rgb]{ 1,  0,  0}{0.121} & \textcolor[rgb]{ 1,  0,  0}{0.811} & 37.501 \\
    % \bottomrule
    \hline
    \hline
    \end{tabular}%
  % }
  \label{tab:ablation_patch}%
\end{table}%

==> tables/L1_DIV2K.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htp]
  \centering
    \footnotesize
    \renewcommand\arraystretch{1.1}
    \setlength{\tabcolsep}{1.4pt}
    \begin{tabular}{c|c|ccccc}
    \hline
    \hline
    \multicolumn{1}{l|}{Test Set} & Loss & PSNR$\uparrow$  & LPIPS$\downarrow$ & DISTS$\downarrow$ & SSIM$\uparrow$  & FID$\downarrow$\\
    \hline
    \multirow{9}{*}{Set5} & L1    & 23.066  & 0.450  & 0.328  & 0.811  & 57.581  \\
\cline{2-7}          & LPIPS(alex) (0.1) & 21.373  & 0.277  & 0.228  & 0.817  & 40.928  \\
          & LPIPS(alex) (0.01) & 19.666  & 0.431  & 0.333  & 0.759  & 172.385  \\
\cline{2-7}          & CTX (0.1) & 27.297  & 0.099  & 0.097  & 0.918  & 5.188  \\
          & CTX (0.01) & 22.914  & 0.120  & 0.144  & 0.862  & 13.460  \\
\cline{2-7}          & PDL (0.1) & 27.653  & 0.178  & 0.146  & 0.852  & 14.175  \\
          & PDL(0.01) & 26.804  & 0.181  & 0.149  & 0.875  & 13.931  \\
\cline{2-7}          & \textbf{FDL (0.1)} & \textbf{29.019 } & \textbf{0.107 } & \textbf{0.098 } & \textbf{0.925 } & \textcolor[rgb]{ 1,  0,  0}{\textbf{4.009 }} \\
          & \textbf{FDL (0.01)} & \textcolor[rgb]{ 1,  0,  0}{\textbf{32.154 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.095 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.095 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.957 }} & \textbf{4.450 } \\
    \hline
    \multirow{9}{*}{Set14} & L1    & 22.286  & 0.539  & 0.352  & 0.749  & 106.836  \\
\cline{2-7}          & LPIPS(alex) (0.1) & 20.905  & 0.329  & 0.237  & 0.782  & 51.432  \\
          & LPIPS(alex) (0.01) & 19.396  & 0.494  & 0.360  & 0.704  & 232.432  \\
\cline{2-7}          & CTX (0.1) & 25.814  & 0.159  & 0.112  & 0.913  & \textcolor[rgb]{ 1,  0,  0}{7.235 } \\
          & CTX (0.01) & 22.327  & 0.176  & 0.153  & 0.854  & 29.962  \\
\cline{2-7}          & PDL (0.1) & 26.279  & 0.236  & 0.163  & 0.826  & 19.854  \\
          & PDL(0.01) & 25.479  & 0.236  & 0.165  & 0.858  & 14.472  \\
\cline{2-7}          & \textbf{FDL (0.1)} & \textbf{26.948 } & \textbf{0.168 } & \textbf{0.109 } & \textbf{0.922 } & \textbf{8.275 } \\
          & \textbf{FDL (0.01)} & \textcolor[rgb]{ 1,  0,  0}{\textbf{29.383 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.157 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.108 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.965 }} & \textbf{8.973 } \\
    \hline
    \multirow{9}{*}{B100} & L1    & 23.110  & 0.549  & 0.378  & 0.725  & 229.265  \\
\cline{2-7}          & LPIPS(alex) (0.1) & 21.837  & 0.329  & 0.250  & 0.753  & 175.323  \\
          & LPIPS(alex) (0.01) & 20.583  & 0.491  & 0.378  & 0.686  & 389.971  \\
\cline{2-7}          & CTX (0.1) & 26.206  & 0.156  & 0.118  & 0.868  & 20.851  \\
          & CTX (0.01) & 23.397  & 0.171  & 0.150  & 0.825  & 48.058  \\
\cline{2-7}          & PDL (0.1) & 26.554  & 0.227  & 0.173  & 0.800  & 34.974  \\
          & PDL(0.01) & 25.897  & 0.230  & 0.176  & 0.825  & 41.311  \\
\cline{2-7}          & \textbf{FDL (0.1)} & \textbf{26.915 } & \textbf{0.167 } & \textbf{0.117 } & \textbf{0.868 } & \textcolor[rgb]{ 1,  0,  0}{\textbf{18.188 }} \\
          & \textbf{FDL (0.01)} & \textcolor[rgb]{ 1,  0,  0}{\textbf{28.791 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.155 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.116 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.908 }} & \textbf{19.663 } \\
    \hline
    \multirow{9}{*}{Urban100} & L1    & 19.962  & 0.507  & 0.355  & 0.639  & 92.895  \\
\cline{2-7}          & LPIPS(alex) (0.1) & 19.339  & 0.305  & 0.235  & 0.673  & 56.614  \\
          & LPIPS(alex) (0.01) & 17.888  & 0.449  & 0.345  & 0.585  & 199.388  \\
\cline{2-7}          & CTX (0.1) & 23.469  & 0.149  & 0.111  & 0.815  & 12.744  \\
          & CTX (0.01) & 20.528  & 0.160  & 0.150  & 0.754  & 46.750  \\
\cline{2-7}          & PDL (0.1) & 23.750  & 0.225  & 0.163  & 0.716  & 24.561  \\
          & PDL(0.01) & 23.148  & 0.228  & 0.166  & 0.749  & 21.997  \\
\cline{2-7}          & \textbf{FDL (0.1)} & \textbf{24.260 } & \textbf{0.154 } & \textbf{0.105 } & \textbf{0.836 } & \textbf{8.870 } \\
          & \textbf{FDL (0.01)} & \textcolor[rgb]{ 1,  0,  0}{\textbf{26.658 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.139 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.102 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.894 }} & \textcolor[rgb]{ 1,  0,  0}{\textbf{8.862 }} \\
    \hline
    \hline
    \end{tabular}%
    \caption{
    Quantitative comparison of SISR using the NLSN model~\cite{mei2021image} trained with synthetic misaligned DIV2K dataset. Each loss is combined with L1 loss using corresponding weights. The best results are marked in~\textcolor{red}{red}.
    }
  \label{tab:L1_DIV2K}%
\end{table}%


==> tables/L1_DPED.tex <==
\begin{table}[t]
  \centering
    % \small
    \footnotesize
    \renewcommand\arraystretch{1.1}
    \setlength{\tabcolsep}{3.0pt}
    \begin{tabular}{c|ccccc}
    % \toprule
    \hline
    \hline
    Loss & PSNR$\uparrow$  & LPIPS$\downarrow$ & DISTS$\downarrow$ & SSIM$\uparrow$  & FID$\downarrow$ \\
    \hline
    L1    & 21.342 & 0.206 & 0.200 & 0.767 & 144.866 \\
    \hline
    LPIPS(alex) (0.1) & 20.931 & 0.175 & 0.174 & 0.766 & 87.699 \\
    LPIPS(alex) (0.01) & 20.824 & 0.190 & 0.187 & 0.763 & 111.283 \\
    \hline
    CTX (0.1) & \textcolor[rgb]{ 1,  0,  0}{21.763} & 0.134 & 0.148 & 0.787 & 38.779 \\
    CTX (0.01) & 20.958 & 0.167 & 0.174 & 0.768 & 88.338 \\
    \hline
    PDL (0.1) & 20.797 & 0.136 & 0.148 & 0.747 & 78.127 \\
    PDL (0.01) & 20.350 & 0.150 & 0.163 & 0.729 & 89.211 \\
    \hline
    \textbf{FDL (0.1)} & \textbf{20.445} & \textbf{0.151} & \textbf{0.160} & \textbf{0.731} & \textbf{91.006} \\
    \textbf{FDL (0.01)} & \textbf{21.165} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.133}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.140}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.789}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{30.405}} \\
    \hline
    \hline
    \end{tabular}%
    % \vspace{-5pt}
    \caption{
    Quantitative comparison of image enhancement using the SwinIR model~\cite{liangSwinIRImageRestoration2021} trained with DPED dataset~\cite{ignatovDSLRQualityPhotosMobile2017a}.
    }
    % \vspace{-10pt}
  \label{tab:L1_DPED}%
\end{table}%


==> tables/L1_RealSR.tex <==
\begin{table}[t]
  \centering
    % \small
    \footnotesize
    \renewcommand\arraystretch{1.1}
    \setlength{\tabcolsep}{3.0pt}
    \begin{tabular}{c|ccccc}
    % \toprule
    \hline
    \hline
    Loss & PSNR$\uparrow$  & LPIPS$\downarrow$ & DISTS$\downarrow$ & SSIM$\uparrow$  & FID$\downarrow$ \\
    \hline
    L1    & \textcolor[rgb]{ 1,  0,  0}{37.368} & 0.111 & 0.124 & \textcolor[rgb]{ 1,  0,  0}{0.978} & 32.246 \\
    \hline
    LPIPS(alex) (0.1) & 36.954 & 0.096 & 0.105 & 0.976 & 33.766 \\
    LPIPS(alex) (0.01) & 37.354 & 0.106 & 0.121 & \textcolor[rgb]{ 1,  0,  0}{0.978} & 40.976 \\
    \hline
    CTX (0.1) & 35.907 & 0.097 & 0.105 & 0.969 & 48.428 \\
    CTX (0.01) & 36.104 & 0.102 & 0.105 & 0.970 & 49.567 \\
    \hline
    PDL (0.1) & 34.523 & 0.099 & 0.105 & 0.951 & 51.348 \\
    PDL (0.01) & 36.094 & 0.090 & 0.097 & 0.968 & 28.991 \\
    \hline
    \textbf{FDL (0.1)} & \textbf{35.981} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.089}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0.091}} & \textbf{0.967} & \textbf{44.501} \\
    \textbf{FDL (0.01)} & \textbf{36.215} & \textbf{0.092} & \textbf{0.096} & \textbf{0.970} & \textcolor[rgb]{ 1,  0,  0}{\textbf{15.172}} \\
    \hline
    \hline
    \end{tabular}%
    % \vspace{-5pt}
    \caption{
    Quantitative comparison of real-world SISR using the SwinIR~\cite{liangSwinIRImageRestoration2021} model trained with merged real-world dataset.
    }
    % \vspace{-10pt}
  \label{tab:L1_RealSR}%
\end{table}%



==> tables/rebuttal_FDL_eval.tex <==
\begin{table}[h]
  \centering
    \caption{
    Quantitative comparison with FDL metric on DPED.}
    % \small
    \footnotesize
    \renewcommand\arraystretch{1.1}
    \setlength{\tabcolsep}{3.0pt}
    \begin{tabular}{c|ccccc}
    % \toprule
    \hline
    \hline
    Metric & CTX  & LPIPS & PDL & FDL \\
    \hline
    FDL$\downarrow$  & 22.251 & 29.966 & 19.556 & 17.950 \\
    \hline
    \hline
    \end{tabular}%
    % \vspace{-5pt}
    % \vspace{-10pt}
  \label{tab:rebuttal_fdl}%
\end{table}%


==> tables/rebuttal_align_level.tex <==
\begin{table}[h]
  \centering
    \caption{
    Quantitative result on varying misalignment degree.}
    % \small
    \footnotesize
    \renewcommand\arraystretch{1.1}
    \setlength{\tabcolsep}{3.0pt}
    \begin{tabular}{c|ccccc}
    % \toprule
    \hline
    \hline
    Misalignment & PSNR$\uparrow$  & LPIPS$\downarrow$ & DISTS$\downarrow$ & SSIM$\uparrow$  & FID$\downarrow$ \\
    \hline
    Slight   & 27.498 & 0.096 & 0.059 & 0.818 & 5.338 \\
    Significant &  27.354  & 0.104 & 0.065 & 0.822 & 5.566 \\
    \hline
    \hline
    \end{tabular}%
    % \vspace{-5pt}
    % \vspace{-10pt}
  \label{tab:rebuttal_wave}%
\end{table}%

==> tables/rebuttal_burstSR.tex <==
\begin{table}[h]
  \centering
    \caption{
    Quantitative result of FDL on BurstSR dataset.}
    % \small
    \footnotesize
    \renewcommand\arraystretch{1.1}
    \setlength{\tabcolsep}{3.0pt}
    \begin{tabular}{c|ccccc}
    % \toprule
    \hline
    \hline
    Loss & PSNR$\uparrow$  & LPIPS$\downarrow$ & DISTS$\downarrow$ & SSIM$\uparrow$  & FID$\downarrow$ \\
    \hline
    L1    & 47.168 & 0.082 & 0.123 & 0.981 & 21.892 \\
    L1 + FDL (0.001) & 46.476 & 0.077 & 0.099 & 0.978 & 21.665 \\ 
    \hline
    \hline
    \end{tabular}%
    % \vspace{-5pt}
    % \vspace{-10pt}
  \label{tab:rebuttal_burstSR}%
\end{table}%


==> tables/rebuttal_wave.tex <==
\begin{table}[h]
  \centering
    \caption{
    Quantitative result of FDL (wavelet) on DPED.}
    % \small
    \footnotesize
    \renewcommand\arraystretch{1.1}
    \setlength{\tabcolsep}{3.0pt}
    \begin{tabular}{c|ccccc}
    % \toprule
    \hline
    \hline
    Loss & PSNR$\uparrow$  & LPIPS$\downarrow$ & DISTS$\downarrow$ & SSIM$\uparrow$  & FID$\downarrow$ \\
    \hline
    FDL (wavelet)    & 22.492 & 0.119 & 0.129 & 0.789 & 73.468 \\
    \hline
    \hline
    \end{tabular}%
    % \vspace{-5pt}
    % \vspace{-10pt}
  \label{tab:rebuttal_wave}%
\end{table}%

